GraphFM: Graph Factorization Machines for Feature Interaction Modeling

Factorization machine (FM) is a prevalent approach to modeling pairwise (second-order) feature interactions when dealing with high-dimensional sparse data. However, on the one hand, FM fails to capture higher-order feature interactions suffering from combinatorial expansion. On the other hand, taking into account interactions between every pair of features may introduce noise and degrade prediction accuracy. To solve the problems, we propose a novel approach, Graph Factorization Machine (GraphFM), by naturally representing features in the graph structure. In particular, we design a mechanism to select the beneficial feature interactions and formulate them as edges between features. Then the proposed model, which integrates the interaction function of FM into the feature aggregation strategy of Graph Neural Network (GNN), can model arbitrary-order feature interactions on the graph-structured features by stacking layers. Experimental results on several real-world datasets have demonstrated the rationality and effectiveness of our proposed approach. The code and data are available at https://github.com/CRIPAC-DIG/GraphCTR}{https://github.com/CRIPAC-DIG/GraphCTR

==> mir-sample-bib.tex <==
\begin{thebibliography}{9}



\bibitem{he2017neural1} B. Ran, D. E. Boyce. {\sl Modeling Dynamic Transportation Network}, Berlin, Germany: Springer-Verlag, pp. 69-83,1996. (Book style)

\bibitem{bib2} G. O. Young. Synthetic structure of industrial plastics. Plastics, 2nd ed., J. Peters, Ed., New York, USA: McGraw-Hill, pp. 15-64, 1964. (Book style with paper title and editor)

\bibitem{bib3} L. C. Su, F. Zhu. Design of a novel omnidrectional stereo vision system. {\sl Acta Automatica Sinica}, vol. 32, no. 1, pp. 67-72, 2006. (in Chinese) (Periodical style)

\bibitem{bib4} R. Roychoudhury, S. Bandyopadhyay, K. Paul. Adistributed mechanism for topology discovery in ad hoc wireless networks using mobile agents. In {\sl Proceedings of IEEE First Annual Workshop on Mobile and Ad hoc Networking and Computing}, IEEE, Piscataway, USA, pp. 145-146,2000. (Published Conference Proceedings style)

\bibitem{bib5} O. Hryniewicz. An evaluation of the reliability of complex systems using shadowed sets and fuzzy lifetime data. {\sl International Journal of Automation and Computing}, to be published.

\bibitem{bib6} W. Zhang. Reinforcement Learning for Job-shop Scheduling, Ph. D. dissertation, Oregon State University, USA,1996. (Dissertation style)

\bibitem{bib7} IEEE Criteria for Class IE Electric Systems, IEEE Standard 308, 1969. (Standards style)

\bibitem{bib8} R. C. Reily, J. L. Mack. The Self-organization of Spatially Invariant Representations, Technical Report PDP. CNS.92.5, Department of Psychology, Mellon University, USA, 1993. (Report style)

\bibitem{bib9} J. P. Wilkinson. Nonlinear Resonant Circuit Devices, U.S. Patent 362412, July 1990. (Patent style)

\bibitem{bib10} J. Jones. {\sl Networks}, 2nd ed., [Online], Available: http://www.atm.com, May 10, 1991.

\bibitem{bib11} R. J. Vidmar. On the use of atmospheric plasmas as electromagnetic reflectors. {\sl IEEE Transactions on Plasma Science}, vol. 21, no. 3, pp. 945-999, [Online], Available: http://www.halcyon.com, July 20-25, 1999.



\end{thebibliography}


